What do we study when studying politics and democracy? A semantic analysis of how politics and democracy are treated in SIGCHI conference papers

Human-computer interaction scholars are increasingly touching on topics related to politics or democracy. As these concepts are ambiguous, an examination of concepts' invoked meanings aids in the self-reflection of our research efforts. We conduct a thematic analysis of all papers with the word `politics' in abstract, title or keywords ($n$=378) and likewise 152 papers with the word `democracy.' We observe that these words are increasingly being used in human-computer interaction, both in absolute and relative terms. At the same time, we show that researchers invoke these words with diverse levels of analysis in mind: the early research focused on mezzo-level (i.e., small groups), but more recently the work has begun to include macro-level analysis (i.e., society and politics as played in the public sphere). After the increasing focus on the macro-level, we see a transition towards more normative and activist research, in some areas it replaces observational and empirical research. These differences indicate semantic differences, which -- in the worst case -- may limit scientific progress. We bring these differences visible to help in further exchanges of ideas and human-computer interaction community to explore how it orients itself to politics and democracy.

==> classification_schema.tex <==
%\begin{tabular}{p{.1\textwidth}p{.62\textwidth}p{.13\textwidth}p{.15\textwidth}}

\toprule
Category & Description & Papers & Keywords \\
\midrule

\endfirsthead

\toprule
\multicolumn{4}{l}{\emph{Table \ref{tab:rq1result}: \nameref{tab:rq1result} continues.}} \\
Category & Description & Papers & Keywords \\
\midrule
\endhead

\midrule
\multicolumn{4}{l}{\emph{Continued on next page}} \\
\bottomrule
\endfoot

\bottomrule
\endlastfoot

  Academic community-building &
  Publications focused on bringing like-minded academics together to discuss research and activities.
  One example is reporting on panel discussions and workshops held as part of academic conferences.
  As with doctoral consortium papers, the focus is on bringing junior scholars into the community, often without statement of specific research outcomes.  % `doctoral students' seminar papers'? -als
  While these papers can be placed in other categories by topic,
  we chose to highlight them as a separate group because they hold a specific purpose for the SIGCHI community. & \multicolumn{2}{p{.3\columnwidth}}{ {\fontsize{3}{4}\selectfont\citepreview{10.1145.2998581.2998616,10.1145.2998581.2998622,10.1145.3004323.3005689,10.1145.2909132.2927472,10.1145.1640233.1640302,10.1145.286498.286538,10.1145.634067.634129,10.1145.506443.506548,10.1145.506443.506649,10.1145.765891.765934,10.1145.1056808.1057110,10.1145.1125451.1125762,10.1145.1125451.1125517,10.1145.1240866.1241088,10.1145.1358628.1358971,10.1145.1520340.1520731,10.1145.1520340.1520472,10.1145.1753846.1753936,10.1145.1753846.1753940,10.1145.1979742.1979568,10.1145.1979742.1979543,10.1145.1979742.1979493,10.1145.2212776.2212715,10.1145.2212776.2212427,10.1145.2559206.2579405,10.1145.2559206.2559227,10.1145.2702613.2702656,10.1145.2702613.2702657,10.1145.2702613.2702616,10.1145.2702613.2702623,10.1145.2702613.2702617,10.1145.2702613.2727687,10.1145.2851581.2912563,10.1145.2851581.2856499,10.1145.2851581.2886436,10.1145.2851581.2886427,10.1145.2851581.2886426,10.1145.3027063.3056455,10.1145.3027063.3027138,10.1145.3027063.3027076,10.1145.3027063.3049280,10.1145.1120212.1120338,10.1145.2793107.2810282,10.1145.2793107.2810283,10.1145.1031607.1031618,10.1145.1958824.1958827,10.1145.2145204.2145206,10.1145.2441776.2441779,10.1145.2818052.2874353,10.1145.2818052.2855505,10.1145.3022198.3022656,10.1145.3022198.3024948,10.1145.3022198.3024945,10.1145.2556420.2556828,10.1145.2685553.2685556,10.1145.2685553.2699325,10.1145.2908805.2913020,10.1145.2908805.2913027,10.1145.3064857.3064860,10.1145.2598784.2598795,10.1145.2598784.2611381,10.1145.2957276.2996292,10.1145.2957276.2997020,10.1145.2631775.2631813,10.1145.2451176.2451230,10.1145.2971485.2987678,10.1145.2971485.2987683,1795316,1795315,1795313,10.1145.601798.601814,10.1145.49108.1046381,10.1145.3024969.3025041,10.1145.1864431.1864502,10.1145.2494091.2495993,10.1145.2800835.2801659,10.1145.2800835.2812801,10.1145.1622176.1622211,10.1145.3131785.3131845} } } \\
  Proceedings & Conference chair's and paper chair's welcome messages in conference proceedings volumes, along with reviews of conferences. &
  {\fontsize{3}{4}\selectfont\citepreview{10.1145.2851581.2912558,10.1145.202642.202651,10.1145.379106.379112,2882850,3025453,2145204,1463689,506443,1880071,2389176,2441776,1999030,1858171,2556420,2998181,2103354} } & \\

  \midrule
  Meta level &
  A category spanning numerous types of contribution by the SIGCHI community, including essay-like ones.
  The work might, for example, propose new conceptual tools to aid in design work or be
  motivated by research-through-design efforts or prompted by analysis in other scientific disciplines.
  Similarly, it might articulate design visions and futures \citep{Reeves2016}
  or propose and address a research agenda.
  Some works in this category address theoretical challenges, such as politics in cross-cultural settings,
  or present reviews of several projects for further analysis.
  The unifying factor is that these works seldom engage with a specific problem domain and are aimed rather more at larger contributions within the community.
  Therefore, they are grouped together.
  & {\fontsize{3}{4}\selectfont\citepreview{10.7146.aahcc.v1i1.21198,10.1145.1501750.1501837,10.1145.276755.276761,10.1145.1556460.1556470,10.1145.2556288.2557359,10.1145.2858036.2858505,10.1145.2858036.2858343,10.1145.2858036.2858482,10.1145.3025453.3025490,10.1145.317456.317469,10.1145.1240866.1240885,10.1145.2212776.2223769,10.1145.2559206.2580091,10.1145.2559206.2578864,10.1145.2145204.2145220,10.1145.62266.62275,10.1145.99332.99367,10.1145.192844.193064,10.1145.1858171.1858173,10.1145.2901790.2901861,10.1145.782896.782909,10.1145.2957276.2957311,1367958,10.1145.1746050.1746063,10.1145.1457199.1457216,10.1145.354384.354390,10.1145.2639189.2639250,10.1145.2971485.2993922,10.1145.2838739.2838769,1795250,10.1145.202642.202655,10.1145.2677199.2691608,10.1145.2638728.2641685} }
  & civic engagement, design, society, civic intelligence, ethnography \\
  Methods &
  Work wherein the main contribution is a novel method
  or the evaluation and discussion of existing methods for research.
  For these works, politics and democracy is often taken as
  motivation (as with potential users of a novel method),
  a source of data (as with election tweets),
  an outcome of analysis (as with determination of users' political alignment),
  or an explanation of outcomes (as in reflection on socio-political context).
  & {\fontsize{3}{4}\selectfont\citepreview{10.1145.1690388.1690420,10.1145.365024.365301,10.1145.1357054.1357101,10.1145.1978942.1979106,10.1145.2556288.2557094,10.1145.2702123.2702491,10.1145.2702123.2702176,10.1145.2858036.2858398,10.1145.2858036.2858472,10.1145.3025453.3025535,10.1145.800275.810930,10.1145.800275.810928,10.1145.1125451.1125591,10.1145.1520340.1520361,10.1145.1753846.1754086,10.1145.2212776.2223697,10.1145.2559206.2574795,10.1145.1958824.1958842,10.1145.2441776.2441852,10.1145.2531602.2531607,10.1145.2531602.2531636,10.1145.2818052.2869111,10.1145.2998181.2998259,10.1145.2998181.2998254,10.1145.1394445.1394467,10.1145.3102071.3110575,10.1145.3148330.3148340,10.1145.2631775.2631795,10.1145.2631775.2631777,10.1145.2631775.2631796,10.1145.2700171.2791033,10.1145.2700171.2791058,10.1145.2700171.2794352,10.1145.2914586.2914599,10.1145.3078714.3078727,10.1145.2818346.2820732,10.1145.1463689.1463741,1367984,10.1145.1111449.1111476,10.1145.2449396.2449424,10.1145.2786567.2787135,1795288,10.1145.2645710.2645734,10.1145.2645710.2645740,10.1145.2792838.2800190,10.1145.2365934.2365943,10.1145.2407696.2407705,2367674,10.1145.2806655.2806657,10.1145.2800835.2809508,10.1145.2800835.2804399,10.4108.icst.urb-iot.2014.257282} }
  & Twitter, social media, social networks, sentiment analysis, World Wide Web \\
  Organisations &
  Research that is focused on an organisation or other social entity.
  Some of this research focuses on the information and communication needs in political organisations.
  These include social movements, non-profits, and activist organisations, as well as government entities.
  Other studies focus on the politics within an organisation, making remarks on organisational politics.
  These studies engage in examining the implications of organisational politics and culture for
  interactive systems' development,
  use of technology within the organisation,
  or
  development and application of user-centered design or other design methodologies within organisations.
  While somewhat different in focus --
  the former examining politics as a research context and the latter as an outcome of a deployment --
  both have clear boundaries for the research theme: an organisation.
  & {\fontsize{3}{4}\selectfont\citepreview{10.1145.276755.276783,10.1145.1556460.1556474,10.1145.2103354.2103357,10.1145.2631488.2631498,10.1145.503376.503419,10.1145.1518701.1519014,10.1145.1753326.1753423,10.1145.1753326.1753406,10.1145.2470654.2466262,10.1145.2556288.2557100,10.1145.2702123.2702522,10.1145.2702123.2702441,10.1145.2702123.2702557,10.1145.2858036.2858153,10.1145.2858036.2858326,10.1145.2858036.2858146,10.1145.2858036.2858420,10.1145.3025453.3025637,10.1145.1056808.1056940,10.1145.1979742.1979835,10.1145.1979742.1979671,10.1145.2559206.2581353,10.1145.2559206.2559971,10.1145.2559206.2559974,10.1145.1234772.1234783,10.1145.1460563.1460581,10.1145.1460563.1460646,10.1145.2145204.2145240,10.1145.2441776.2441938,10.1145.2531602.2531664,10.1145.2675133.2675156,10.1145.2675133.2675163,10.1145.2818048.2820031,10.1145.2818048.2819942,10.1145.2818048.2820027,10.1145.3022198.3026317,10.1145.3022198.3026313,10.1145.192844.192869,10.1145.778712.778743,10.1145.2901790.2901848,10.1145.2347504.2347550,10.1145.2660398.2660435,10.1145.2160881.2160886,10.1145.3078072.3079749,1795237,1795238,10.1145.122672.122688,10.1145.30851.275650,10.1145.2493432.2493499,10.1145.2494091.2496042} }
  & activism, social media, politics, ethnography, participatory design \\
  Policy work &
  Works focused on policies and best practices related to human--computer interaction.
  These encompass
  research and review of accessibility regulations,
  teaching of human--computer interaction,
  work on regulation and policy decisions related to infrastructure,
  and
  empirical and philosophical discussions of privacy in online environments.
  The category also includes discussion of science policy, such as funding arrangements and evaluations of human--computer interaction as a scientific enterprise.
  & {\fontsize{3}{4}\selectfont\citepreview{10.1145.276755.276774,10.1145.276755.276785,10.1145.276758.276778,10.1145.2466627.2485921,10.1145.2103354.2103371,10.1145.1753326.1753689,10.1145.2556288.2557261,10.1145.3025453.3025961,10.1145.765891.765950,10.1145.985921.985963,10.1145.2559206.2578880,10.1145.2901790.2901882,10.1145.3125739.3125758,2729531,1999635,10.1145.1148613.1148615,10.1145.357744.357919,10.1145.157203.157205,10.1145.214132.214168,10.1145.67900.67901,10.1145.198125.198127,10.1145.1015528.810926,10.1145.2638728.2641681,10.1145.2638728.2641309,10.1145.1969289.1969310,10.1145.2207016.2207028} }
  & accessibility, e-government, privacy, social change, EULA \\
  Public service delivery &
  Work on how technology can improve the delivery of governmental or public services.
  The papers focus on specific domains of public services, such as health-care or social services,
  or on certain user groups, such as migrants, homeless people, or users who face accessibility challenges.
  These works range from empirical investigations of current situations to constructive work proposing new and alternative systems for public service delivery.
  Furthermore, some of them examine how public organisations (and non-profit organisations providing services of public value) implement technology-based services to support their efforts to deliver their services.
  & {\fontsize{3}{4}\selectfont\citepreview{10.7146.aahcc.v1i1.21315,10.7146.aahcc.v1i1.21297,10.1145.2998581.2998610,10.1145.1842993.1843082,10.1145.2254556.2254568,10.1145.1753326.1753610,10.1145.2207676.2208342,10.1145.2556288.2556971,10.1145.2702123.2702157,10.1145.2702123.2702324,10.1145.2858036.2858331,10.1145.2858036.2858105,10.1145.3025453.3025968,10.1145.3025453.3025931,10.1145.3025453.3025943,10.1145.3025453.3025881,10.1145.3025453.3025983,10.1145.765891.765964,10.1145.2559206.2581270,10.1145.2702613.2732893,10.1145.2851581.2851586,10.1145.3027063.3052764,10.1145.3020165.3022175,10.1145.2441776.2441832,10.1145.2531602.2531712,10.1145.960201.957208,10.1145.1013115.1013176,10.1145.1394445.1394486,10.1145.1858171.1858174,2729542,2254518,10.1145.2676702.2677201,10.1145.2557500.2557513,10.1145.2071536.2071555,1795306,10.4108.icst.pervasivehealth.2014.255783,10.1145.2370216.2370469,10.1145.2971648.2971731,10.1145.2461121.2461131} }
  & e-government, design, civic engagement, participatory design, feedback \\
  Political communication &
  Research focusing on the use of information and communication technologies for distributing and exchanging political views.
  Most works in this category focus on empirical investigation of social media,
  whether addressing general use (wherein political communication is one of the factors)
  or examining political events or actors, such as social media use during elections, second-screening activities, or politicians' use of social media.
  Some of the papers focus on proposing and developing alternative ways to display this information,
  with a minority of the works being focused on other forms of political information dissemination, such as
  reflection on how games can be used for sharing political views or on
  analysis of politically oriented Web sites and their features.
  & {\fontsize{3}{4}\selectfont\citepreview{10.1145.2523429.2523456,10.1145.2254556.2254644,10.1145.1357054.1357304,10.1145.2470654.2470659,10.1145.2556288.2557197,10.1145.2702123.2702193,10.1145.2702123.2702291,10.1145.2858036.2858423,10.1145.2858036.2858160,10.1145.3025453.3025611,10.1145.3025453.3025543,10.1145.3025453.3025833,10.1145.1358628.1358925,10.1145.1520340.1520446,10.1145.1520340.1520574,10.1145.2212776.2223843,10.1145.3027063.3053185,10.1145.3130859.3131434,10.1145.2145204.2145213,10.1145.2145204.2145212,10.1145.2441776.2441876,10.1145.2441776.2441935,10.1145.2531602.2531719,10.1145.2531602.2531735,10.1145.2675133.2675187,10.1145.2818048.2820004,10.1145.2818052.2874318,10.1145.2818052.2893359,10.1145.2998181.2998295,10.1145.2998181.2998340,10.1145.2998181.2998194,10.1145.2079216.2079254,10.1145.1413634.1413734,10.1145.1858171.1858232,10.1145.3102071.3102101,10.1145.2389176.2389233,10.1145.3148330.3152697,10.1145.3148330.3148336,2729508,10.1145.2631775.2631788,10.1145.2631775.2631823,10.1145.2700171.2791056,10.1145.2914586.2914665,10.1145.3078714.3078736,10.1145.1841853.1841876,10.1145.2181037.2181088,10.1145.2037373.2037437,10.1145.2971485.2971514,10.1145.2757710.2757733,10.1145.2602299.2602308,10.1145.2745197.2755521,10.1145.2494091.2499225,10.1145.3099023.3099055} }
  & social media, politics, Twitter, television, civic engagement \\
  Supporting diversity and reducing bias &
  A stream of research focused on biases, polarisation, selective exposure, and fact-checking.
  The topics include analysis centered on news outlets
  (such as discussion and sharing of news stories via social media)
  and work to analyse and make proposals for avoiding media bias in the selection of news outlets to follow.
  Works for which the aim was to increase diversity in social-media followership belong to this class if their focus is on similar literature, even when the emphasis is not on news outlets.
  & {\fontsize{3}{4}\selectfont\citepreview{10.1145.1518701.1518772,10.1145.1518701.1518824,10.1145.1753326.1753541,10.1145.1753326.1753543,10.1145.1978942.1979127,10.1145.2858036.2858510,10.1145.1520340.1520552,10.1145.3027063.3053227,10.1145.2441776.2441895,10.1145.2441776.2441877,10.1145.2531602.2531676,10.1145.2818052.2874354,10.1145.2998181.2998287,10.1145.2700171.2791057,10.1145.3078714.3078724,10.1145.2856767.2856776} }
  & politics, social media, media bias, credibility, presentation \\
  Supporting neighborhoods &
  A category of work via which researchers seek to analyse and produce tools with which neighbourhood or hyperlocal communities can be supported via technology.
  These range from social-media tools used to organise community actions
  to application of public screens to reflect what is taking place in the community and increase its social cohesion.
  & {\fontsize{3}{4}\selectfont\citepreview{10.1145.2757226.2757369,10.1145.2470654.2466478,10.1145.2556288.2557319,10.1145.2556288.2557054,10.1145.2468356.2468420,10.1145.2468356.2468837,10.1145.2559206.2581354,10.1145.2702613.2732777,10.1145.3027063.3049273,10.1145.2531602.2531714,10.1145.2675133.2675182,10.1145.2818048.2819985,10.1145.2685553.2699016,10.1145.2598510.2598563,10.1145.3064663.3064723,10.1145.3064663.3064751,1138289,10.1145.2686612.2686627,10.1145.2370216.2370401,10.1145.2494091.2496004} }
  & civic engagement, social media, community, participatory design, citizen engagement \\
  Supporting participation &
  Research that examines the potential of information and communication technology to support participation in decision-making.
  The focus of activity here is on
  participation at local level;
  non-political participation, such as participation at schools;
  and online tools for participation on a large scale, such as e-petition sites or news-commenting systems.
  Relative to articles in other classes (such as supporting neighborhoods, public service delivery, or political communication), these papers make clearer reference to decision-making.
  % This literature is further examined in Section~\ref{rq2}.
  & {\fontsize{3}{4}\selectfont\citepreview{10.1145.1385569.1385652,10.1145.2598153.2598202,10.1145.2757226.2757236,10.1145.1556460.1556492,10.1145.2103354.2103367,10.1145.2103354.2103362,10.1145.1518701.1518762,10.1145.1978942.1979290,10.1145.2207676.2208621,10.1145.2207676.2208594,10.1145.2470654.2470770,10.1145.2470654.2470714,10.1145.2702123.2702559,10.1145.2702123.2702403,10.1145.2702123.2702255,10.1145.2702123.2702558,10.1145.2702123.2702352,10.1145.2858036.2858429,10.1145.2858036.2858098,10.1145.2858036.2858332,10.1145.3025453.3025963,10.1145.3025453.3025885,10.1145.3025453.3025559,10.1145.3025453.3025996,10.1145.3025453.3026034,10.1145.3025453.3025897,10.1145.985921.986190,10.1145.1056808.1057014,10.1145.1753846.1753898,10.1145.1753846.1753872,10.1145.1979742.1979852,10.1145.1979742.1979869,10.1145.2468356.2479538,10.1145.2702613.2725432,10.1145.3027063.3053265,10.1145.3027063.3052549,10.1145.3027063.3053248,10.1145.3130859.3131338,10.1145.2145204.2145239,10.1145.2145204.2145244,10.1145.2145204.2145251,10.1145.2145204.2145249,10.1145.2531602.2531677,10.1145.2531602.2531605,10.1145.2531602.2531639,10.1145.2675133.2675134,10.1145.2675133.2675212,10.1145.2818052.2869125,10.1145.2998181.2998235,10.1145.2998181.2998291,10.1145.3022198.3026358,10.1145.2556420.2556785,10.1145.1858171.1858175,10.1145.1858171.1858208,10.1145.2317956.2317980,10.1145.2317956.2317982,10.1145.2598510.2598534,10.1145.2598510.2598523,10.1145.2901790.2901877,10.1145.3064663.3064684,10.1145.3064857.3079111,10.1145.3064857.3079113,10.1145.997078.997092,1138241,10.1145.1463689.1463704,10.1145.1941007.1941042,10.1145.2992154.2992163,10.1145.2817721.2817734,10.1145.1499224.1499273,10.1145.1457199.1457229,10.1145.1152215.1152285,10.1145.2935334.2935379,10.1145.2399016.2399046,10.1145.2838739.2838759,1795273,1795318,1795298,10.1145.2611009.2611029,10.1145.2611009.2611015,10.1145.2898365.2899799,10.1145.2745197.2755518,10.1145.1864349.1864358,10.1145.2370216.2370399,10.1145.2370216.2370221,10.1145.2494091.2495994,10.1145.2494091.2495995,10.1145.2800835.2804403,10.1145.2800835.2804400,10.1145.2800835.2801622,10.1145.2800835.2804401} }
  & civic engagement, deliberation, participatory design, design, voting \\
  Technology democratization &
  Research focused on the increased access to or benefits of technology that arise from, for example,
  decreased costs and
  increased simplicity.
  Beyond traditional focus on the digital divide, these papers also examine
  democratization due to access to
  visualization tools,
  knowledge,
  manufacturing tools,
  and changes in roles (such as consumer and producer).
  & {\fontsize{3}{4}\selectfont\citepreview{10.1145.1690388.1690493,10.1145.2909132.2909249,10.1145.1640233.1640309,10.1145.1640233.1640270,10.1145.2069618.2069665,10.1145.1254960.1254999,10.1145.1357054.1357102,10.1145.1753326.1753393,10.1145.2207676.2208378,10.1145.2470654.2481360,10.1145.2556288.2557221,10.1145.2702123.2702235,10.1145.2858036.2858506,10.1145.2858036.2858059,10.1145.2858036.2858575,10.1145.3025453.3025853,10.1145.29933.275654,10.1145.1958824.1958929,10.1145.2675133.2675195,10.1145.2998181.2998265,10.1145.2998181.2998239,10.1145.1013115.1013136,10.1145.2317956.2318085,10.1145.2598510.2598566,10.1145.3064663.3064674,10.1145.3064663.3064748,10.1145.2607023.2611454,10.1145.2957276.2996281,10.1145.2663204.2669986,10.1145.2820619.2820620,10.1145.3132272.3132299,10.1145.2076354.2076393,10.1145.2876456.2879482,10.1145.3025171.3025227,10.1145.2181037.2181091,10.1145.2393132.2393142,10.1145.2493190.2493205,10.1145.2935334.2935352,10.1145.1868914.1868937,10.1145.1868914.1868925,10.1145.2399016.2399161,10.1145.2414536.2414594,10.1145.2491568.2491595,10.1145.1517664.1517743,10.1145.1935701.1935758,10.1145.2540930.2540933,10.1145.2839462.2872960,10.1145.2370216.2370293,10.1145.2494091.2496000,10.1145.2968219.2971435} }
  & DIY, ubiquitous computing, design, democratization, HCI \\
  Values &
  Papers engaging with questions of values and technology.
  They may take traditional science and technology studies perspectives, considering
  how technical systems and infrastructure can come with certain values or
  offering critical reflection on established systems and practices.
  They may also examine methods that address values in human--computer interaction work, as with application of participatory design approaches or other design methods that focus on understanding values.
  & {\fontsize{3}{4}\selectfont\citepreview{10.1145.276755.276762,10.1145.3059454.3059495,10.1145.1054972.1055076,10.1145.1753326.1753465,10.1145.1978942.1979003,10.1145.2470654.2466152,10.1145.2470654.2481350,10.1145.2556288.2557196,10.1145.2702123.2702298,10.1145.2858036.2858181,10.1145.2858036.2858592,10.1145.2858036.2858151,10.1145.3025453.3026031,10.1145.800049.801757,10.1145.2468356.2468739,10.1145.2468356.2468777,10.1145.2559206.2581358,10.1145.2851581.2856470,10.1145.3027063.3052760,10.1145.2793107.2810259,10.1145.2531602.2531692,10.1145.2675133.2697079,10.1145.2675133.2675282,10.1145.2818048.2820026,10.1145.2818048.2819952,10.1145.2998181.2998321,10.1145.2998181.2998209,10.1145.2556420.2556511,10.1145.1555619.1555638,10.1145.1394445.1394480,10.1145.3064857.3079141,10.1145.997078.997117,10.1145.3102071.3110573,10.1145.1841853.1841906,10.1145.3078072.3079725,10.1145.3123021.3123073,10.1145.1930488.1930498,10.1145.1377999.1378049,10.1145.1868914.1869007,10.1145.2399016.2399116,10.1145.2971485.2996748,10.1145.2686612.2686623,1795305,1795245,1795249,1795248,10.4108.icst.pervasivehealth.2013.252060,10.4108.icst.pervasivehealth.2014.255433,10.1145.1935701.1935773,10.1145.2494091.2499623} }
  & design, participatory design, ethnography, values, activism \\
  \hline

  Other work &
  \multicolumn{3}{l}{
 {\fontsize{3}{4}\selectfont\citepreview{10.1145.2556288.2557311,10.1145.3025453.3025915,10.1145.3025453.3025647,10.1145.3025453.3025948,10.1145.3025453.3025615,10.1145.2531602.2531611,10.1145.2818052.2869132,10.1145.2901790.2901825,10.1145.2347504.2347548,10.1145.1378773.1378786,10.1145.1930488.1930534,10.1145.2935334.2935354,10.1145.3024969.3024971,10.1145.2494091.2495997} }
 } \\


%\end{tabular}


==> democracy_models.tex <==
\begin{threeparttable}

	\centering
	\begin{tabular}{@{}lrrrl@{}}
		\toprule
& \multicolumn{1}{l}{Citizen-driven} & \multicolumn{1}{l}{Organization-lead} & \multicolumn{1}{c}{Total} & \multicolumn{1}{c}{Examples} \\
\midrule
Representative & 2 & 7 & 9 & \citet{10.1145.1753846.1753872,10.1145.997078.997092} \\
Referendum & 8 & 29 & 37 & \citet{10.1145.2858036.2858429,10.1145.2858036.2858098} \\
Assembly & 28 & 26 & 54 & \citet{10.1145.1979742.1979869,10.1145.2145204.2145239} \\
\midrule
\multicolumn{1}{c}{Total} & 38 & 62 & 100 &\\
\multicolumn{1}{c}{Examples} & \citep{10.1145.2145204.2145239} & \citep{10.1145.2858036.2858429} & &\\ %%
\bottomrule
\end{tabular}

\begin{tablenotes} \begin{tiny}
	\item One paper could be classified as belonging to more than one type of democracy or to support both citizen-driven or organisation-led activities, i.e., classes are not exclusive. Furthermore, some papers did not make explicit reference to the form of democracy (Representative, Referendum or Asssembly) supported in the paper. Examples chosen to present a few prominent cases.
\end{tiny} \end{tablenotes}

\caption{Approach to democracy in papers part of the literature (\%)}
\label{tab:rq2democracy}

\end{threeparttable}


==> research_problem.tex <==
\begin{threeparttable}

\centering
\begin{tabular}{@{}lrrrr|rrrl@{}}
\toprule
& \rotatebox[origin=l]{90}{Representative} & \rotatebox[origin=l]{90}{Referedum} & \rotatebox[origin=l]{90}{Assembly} & \multicolumn{1}{c}{Total} & \rotatebox[origin=l]{90}{Citizen-driven} & \rotatebox[origin=l]{90}{Organization-lead} & \multicolumn{1}{c}{Total} & \multicolumn{1}{c}{Examples}  \\
\midrule
Constructive & 3 & 17 & 24 & 44 & 14 & 28 & 42 & \citet{10.1145.1556460.1556492} \\
Empirical & 6 & 19 & 30 & 55 & 25 & 32 & 57 & \citet{10.1145.3022198.3026358}  \\
Conceptual & 0 & 1 & 0 & 1 & 0 & 1 & 1 & \citet{10.1145.2494091.2495995} \\
\midrule
Total & 9 & 37 & 54 & 100 & 39 & 61 & 100 &  \\
\bottomrule
\end{tabular}

\begin{tablenotes} \begin{tiny}
\item See Table~\ref{tab:rq2democracy} for notes.
\end{tiny} \end{tablenotes}

\caption{Research problems in papers part of the literature (\%)}
\label{tab:rq2research}

\end{threeparttable}

